ReLight My NeRF: A Dataset for Novel View Synthesis and Relighting of Real World Objects

In this paper, we focus on the problem of rendering novel views from a Neural Radiance Field (NeRF) under unobserved light conditions. To this end, we introduce a novel dataset, dubbed ReNe (Relighting NeRF), framing real world objects under one-light-at-time (OLAT) conditions, annotated with accurate ground-truth camera and light poses. Our acquisition pipeline leverages two robotic arms holding, respectively, a camera and an omni-directional point-wise light source. We release a total of 20 scenes depicting a variety of objects with complex geometry and challenging materials. Each scene includes 2000 images, acquired from 50 different points of views under 40 different OLAT conditions. By leveraging the dataset, we perform an ablation study on the relighting capability of variants of the vanilla NeRF architecture and identify a lightweight architecture that can render novel views of an object under novel light conditions, which we use to establish a non-trivial baseline for the dataset. Dataset and benchmark are available at https://eyecan-ai.github.io/rene.

==> results/reb_ablation.tex <==
\begin{table}
    \resizebox{\linewidth}{!}{
      \centering
       \setlength{\tabcolsep}{1.5mm}
      {\small
       \begin{tabular}{l|cccccccc}
       \toprule
       Method & \multicolumn{2}{c}{Cube} & \multicolumn{2}{c}{Savannah} & \multicolumn{2}{c}{Reflective} & \multicolumn{2}{c}{FlipFlop} \\
       \midrule
       &  PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\  
       \midrule
       NeRF-Instant & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
       NeRF-Instant learned light & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
       \bottomrule
      \end{tabular}
      }
   }
  %\vspace{3mm}
  \caption{\label{tab:architecture_crop}}
\end{table}


==> results/reb_crop_ablation.tex <==
\begin{table}
    \caption{\label{tab:architecture_crop} Results on cropped images from the validation set.}
    \vspace{-2mm}
    \centering
    \resizebox{0.8\linewidth}{!}{
       \setlength{\tabcolsep}{1.5mm}
      {\small
       \begin{tabular}{l|cccccccc}
       \toprule
       Method & \multicolumn{2}{c}{Cube} & \multicolumn{2}{c}{Savannah} & \multicolumn{2}{c}{Reflective} & \multicolumn{2}{c}{FlipFlop} \\
       \midrule
       & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\  
       \midrule
       V1 & 23.75 & 0.52 & 20.87 & 0.43 & 21.72 & 0.53 & 22.51 & 0.54 \\
       V2 & 23.96 & 0.53 & 22.51 & 0.52 & 21.94 & 0.54 & 23.33 & 0.58 \\
       V3 & 25.32 & 0.60 & 23.54 & 0.57 & 23.69 & 0.61 & 24.11 & 0.60 \\
       V4 & 25.01 & 0.58 & 23.83 & 0.59 & 23.01 & 0.59 & 24.07 & 0.60 \\
       V5 & \textbf{25.64} & \textbf{0.64} & \textbf{24.11} & \textbf{0.62} & \textbf{23.99} & \textbf{0.63} & \textbf{24.33} & \textbf{0.62} \\
       \bottomrule
      \end{tabular}
      }
   }
  \vspace{-7mm}
\end{table}







==> results/reb_relight_instant.tex <==
\begin{table}
    \centering
    \resizebox{0.7\linewidth}{!}{
       \setlength{\tabcolsep}{1.5mm}
      {\small
       \begin{tabular}{l|cc|cc}
       \toprule
       \multicolumn{1}{c}{Name} & \multicolumn{2}{c}{\textit{Easy}} & \multicolumn{2}{c}{\textit{Hard}} \\
       \midrule
       & PSNR & SSIM & PSNR & SSIM \\       
       \hline                     
       Apple & 20.89 & 0.45 & 20.95 & 0.45 \\  
       Cheetah & 19.37 & 0.44 & 19.60 & 0.44 \\  
       Cube & 20.14 & 0.42 & 20.31 & 0.42 \\  
       Dinosaurs & 19.58 & 0.42 & 19.66 & 0.41 \\  
       FlipFlop & 20.38 & 0.45 & 20.36 & 0.45 \\ 
       Fruits & 20.16 & 0.45 & 20.21 & 0.44 \\  
       Garden & 19.76 & 0.45 & 19.70 & 0.45 \\  
       Helicopters  & 19.34 & 0.37 & 19.27 & 0.37 \\  
       Kittens & 18.52 & 0.37 & 18.65 & 0.37 \\  
       Lego & 20.75 & 0.46 & 20.76 & 0.46 \\  
       Lunch & 19.32 & 0.46 & 19.38 & 0.45 \\  
       Plant & 20.62 & 0.44 & 20.66 & 0.44 \\  
       Reflective & 20.09 & 0.43 & 20.11 & 0.42 \\  
       Robotoy & 20.77 & 0.50 & 20.78 & 0.50 \\  
       Savannah & 19.08 & 0.40 & 19.18 & 0.40 \\  
       Shark & 20.54 & 0.42 & 20.53 & 0.41 \\  
       Stegosaurus & 20.84 & 0.43 & 20.91 & 0.42 \\  
       Tapes & 19.34 & 0.41 & 19.55 & 0.41 \\         
       Trucks & 19.81 & 0.44 & 19.87 & 0.44 \\     
       Wooden toys & 20.19 & 0.48 & 20.22 & 0.48 \\   
       \midrule
       Average & 0 & 0 & 0 & 0 \\
       \bottomrule
      \end{tabular}
      }
   }
  %\vspace{3mm}
  \caption{\label{tab:relight_instant} Quantitative results for InstantNGP method across all 20 scenes. We measured both Peak Signal-to-Noise Ratio (PSNR), on the left column, and Structural Similarity (SSIM), on the right column, by comparing the novel view synthetized image with its corresponding groundtruth.}
\end{table}



==> results/reb_relight_optimized_pose.tex <==
\begin{table}
    \caption{\label{tab:relight_opt_pose} Results on \textbf{hardtest} optimizing the light pose.}
    \vspace{-2mm}
    \centering
    \resizebox{0.8\linewidth}{!}{
       \setlength{\tabcolsep}{1.5mm}
      {\small
       \begin{tabular}{l|cccccccc}
       \toprule
       Method & \multicolumn{2}{c}{Cube} & \multicolumn{2}{c}{Savannah} & \multicolumn{2}{c}{Reflective} & \multicolumn{2}{c}{FlipFlop} \\
       \midrule
       & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\  
       \midrule
       V1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
       V2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
       V3 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
       V4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
       V5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
       \bottomrule
      \end{tabular}
      }
   }
  \vspace{-6mm}
\end{table}

==> results/relight.tex <==
\begin{table}
    \centering
    \resizebox{0.7\linewidth}{!}{
       \setlength{\tabcolsep}{1.5mm}
      {\small
       \begin{tabular}{l|cc|cc}
       \toprule
       \multicolumn{1}{c}{Name} & \multicolumn{2}{c}{\textit{Easy}} & \multicolumn{2}{c}{\textit{Hard}} \\
       \midrule
       & PSNR & SSIM & PSNR & SSIM \\       
       \hline                     
       Apple & 26.44 & 0.62 & 26.25 & 0.62 \\  
       Cheetah & 25.66 & 0.61 & 24.64 & 0.60 \\  
       Cube & 24.90 & 0.54 & 23.98 & 0.53 \\  
       Dinosaurs & 25.75 & 0.65 & 24.98 & 0.64 \\  
       FlipFlop & 25.85 & 0.61 & 25.42 & 0.61 \\ 
       Fruits & 25.93 & 0.62 & 25.72 & 0.62 \\  
       Garden & 25.74 & 0.66 & 25.08 & 0.66 \\  
       Helicopters  &  25.12 & 0.61 & 24.73 & 0.61 \\  
       Kittens & 25.90 & 0.64 & 24.96 & 0.63 \\  
       Lego & 26.07 & 0.61 & 25.77 & 0.61 \\  
       Lunch & 25.84 & 0.60 & 24.71 & 0.59 \\  
       Plant & 26.55 & 0.67 & 25.93 & 0.67 \\  
       Reflective & 25.79 & 0.61 & 25.28 & 0.61 \\  
       Robotoy & 26.24 & 0.65 & 25.55 & 0.65 \\  
       Savannah & 25.15 & 0.62 & 24.31 & 0.61 \\  
       Shark & 25.59 & 0.57 & 25.32 & 0.56 \\  
       Stegosaurus & 25.87 & 0.63 & 25.65 & 0.63 \\  
       Tapes & 25.84 & 0.58 & 25.41 & 0.57 \\         
       Trucks & 25.80 & 0.67 & 25.16 & 0.66 \\     
       Wooden toys & 25.69 & 0.61 & 25.24 & 0.60 \\   
       \midrule
       Average & 25.79 & 0.62 & 25.20 & 0.61 \\
       \bottomrule
      \end{tabular}
      }
   }
  %\vspace{3mm}
  \caption{\label{tab:relight} Quantitative results of the V5 method across all 20 scenes. We measured both Peak Signal-to-Noise Ratio (PSNR), on the left column, and Structural Similarity (SSIM), on the right column, by comparing the novel view synthetized image with its corresponding groundtruth.}
\end{table}


